End-to-End Multi-Track Reconstruction using Graph Neural Networks at Belle II

We present the study of an end-to-end multi-track reconstruction algorithm for the central drift chamber of the Belle II experiment at the SuperKEKB collider using Graph Neural Networks for an unknown number of particles. The algorithm uses detector hits as inputs without pre-filtering to simultaneously predict the number of track candidates in an event and their kinematic properties. In a second step, we cluster detector hits for each track candidate to pass to a track fitting algorithm. Using a realistic full detector simulation including beam-induced backgrounds and detector noise taken from actual collision data, we find significant improvements in track finding efficiencies for tracks in a variety of different event topologies compared to the existing baseline algorithm used in Belle II. For events with a hypothetical long-lived massive particle with a mass in the GeV-range decaying uniformly along its flight direction into two charged particles, the GNN achieves a combined track finding and fitting efficiency of 85.4% with a fake rate of 2.5%, compared to 52.2% and 4.1% for the baseline algorithm. This is the first end-to-end multi-track machine learning algorithm for a drift chamber detector that has been utilized in a realistic particle physics environment.

==> nominal.tex <==
\section{Results}\label{sec_results}
In this section we show a comparison of the \cat, the \legendre, the \ca, and the combination of \legendre and \ca with and without the GENFIT2 track fits.
We discuss the track finding efficiency in \cref{sec_results_efficiency}, and the momentum and position resolution in \cref{sec_results_momentum} both for evaluation samples similar to our training samples, but also for simulated physics samples of radiative muon pairs $e^+e^-\to\mu^+\mu^-(\gamma)$, generic samples of $\Upsilon(4S)\to B\bar{B}$ decays, and \kshort from $B^0\to J/\Psi\kshort$ decays.
We then show a detailed analysis of the \cat robustness against different beam backgrounds in training and evaluation in \cref{sec_results_beambackground}, and the \cat ability to generalise to different event topologies not seen during training.

 \subsection{Tracking efficiency}\label{sec_results_efficiency}
Track finding efficiency (see \cref{eq:trackeff}) is dependent on the number of matched signal hits, and the number of beam background hits that are wrongly assigned to the track.
In general, particles that leave a small number of matched signal hits are harder to reconstruct by the track finding algorithms.
This mostly effects particles with very small or very large polar angles in the forward or backward region, particles with small transverse momenta, or particle that are produced at a large distance of the decay vertex from the IP.

\subsubsection{Prompt tracks}
We evaluate the track finding efficiency on events with 1-6 charged particles, $xx < \pgen < xx$, $xx < \thetagen < xx$,  $xx < \phigen < xx$, $\zgen=0$ drawn randomly from independent uniform distributions for each charged particle. \tf{What is the simulated momentum range for the validatin sample?} 
The track finding efficiencies before track fitting, and the combined track finding and track fitting efficiency for the different track finding algorithms in comparison with the \cat are shown in \cref{fig:trainingsample_eff_pt}.
Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate are shown in \cref{tab:trainingsample_low_beambackground} and \cref{tab:trainingsample_high_beambackground}.

\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/test_set/ep3/truth_pt_th_0_35_4_hnum_7_1000__efficiency.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/test_set/ep3/truth_pt_th_35_4_123_4_hnum_7_1000__efficiency.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/test_set/ep3/truth_pt_th_123_4_180_hnum_7_1000__efficiency.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c}
     \end{subfigure}\hfill\\
     
      \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/test_set/np3/truth_pt_th_0_35_4_hnum_7_1000__efficiency.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/test_set/np3/truth_pt_th_35_4_123_4_hnum_7_1000__efficiency.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/test_set/np3/truth_pt_th_123_4_180_hnum_7_1000__efficiency.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c2}
     \end{subfigure}

\caption{Track finding~(empty markers, connected by dashed lines to guide the eye) and combined track finding and fitting efficiency~(filled markers, connected by solid lines to guide the eye) for (top)~low beam background and (bottom)~high beam background as function of transverse momentum $p_t$ for the \legendre~(blue), the \ca~(gray), the combined \legendre+\ca~(purple), and the \cat~(red) in the (\subref{fig:p_eff:a} and \subref{fig:p_eff:a2}) forward endcap, (\subref{fig:p_eff:b} and \subref{fig:p_eff:b2}) barrel, and (\subref{fig:p_eff:c} and \subref{fig:p_eff:c2}) backward endcap.
The errorbars show the statistical uncertainty.
The uncertainties of the different track finding algorithms are correlated since they use the same simulated events.}
\label{fig:trainingsample_eff_pt}
\end{figure*}

\begin{table*}
    \fontsize{8pt}{8pt}\selectfont
    \centering
    \caption{Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate for the evaluation samples for different track finding algorithms in different detector regions for low beam background for the evaluation sample.}
    \begin{tabular}{r ccc ccc ccc}
         \toprule
         & \multicolumn{3}{c}{FWD} &  \multicolumn{3}{c}{Barrel} & \multicolumn{3}{c}{BWD} \\
         & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate\\
         \midrule

%          Legendre & $0.88^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $1.0^{+0.0}_{-0.0}$ & $0.07^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.71^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
% CA + Legendre & $0.95^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $1.0^{+0.0}_{-0.0}$ & $0.1^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.92^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
% CA& $0.97^{+0.0}_{-0.0}$ & $0.03^{+0.0}_{-0.0}$ & $0.06^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.09^{+0.0}_{-0.0}$ & $0.17^{+0.01}_{-0.01}$ & $0.94^{+0.0}_{-0.0}$ & $0.03^{+0.0}_{-0.0}$ & $0.04^{+0.0}_{-0.0}$ \\  \midrule
% CAT & $0.94^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.97^{+0.01}_{-0.0}$ & $0.09^{+0.01}_{-0.01}$ & $0.01^{+0.0}_{-0.0}$ & $0.93^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ \\

Legendre & $0.88^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.71^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
CA + Legendre & $0.95^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.92^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
CA & $0.97^{+0.0}_{-0.0}$ & $0.03^{+0.0}_{-0.0}$ & $0.06^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.03^{+0.0}_{-0.0}$ & $0.17^{+0.0}_{-0.0}$ & $0.94^{+0.0}_{-0.0}$ & $0.03^{+0.0}_{-0.0}$ & $0.04^{+0.0}_{-0.0}$ \\ \midrule
CAT & $0.98^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.97^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.98^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ \\
       
        \bottomrule
    \end{tabular}
    \label{tab:trainingsample_low_beambackground}
\end{table*}

\begin{table*}
    \fontsize{8pt}{8pt}\selectfont
    \centering
    \caption{Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate for the evaluation samples for different track finding algorithms in different detector regions for high beam background for the evaluation sample.}
    \begin{tabular}{r ccc ccc ccc}
         \toprule
         & \multicolumn{3}{c}{FWD} &  \multicolumn{3}{c}{Barrel} & \multicolumn{3}{c}{BWD} \\
         & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate\\
         \midrule
        Legendre & $0.49^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.97^{+0.0}_{-0.0}$ & $0.03^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.3^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
CA + Legendre & $0.77^{+0.0}_{-0.0}$ & $0.21^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.98^{+0.0}_{-0.0}$ & $0.06^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.74^{+0.0}_{-0.0}$ & $0.24^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ \\
CA & $0.91^{+0.0}_{-0.0}$ & $0.41^{+0.0}_{-0.0}$ & $0.17^{+0.0}_{-0.0}$ & $0.98^{+0.0}_{-0.0}$ & $0.15^{+0.0}_{-0.0}$ & $0.41^{+0.0}_{-0.0}$ & $0.81^{+0.0}_{-0.0}$ & $0.47^{+0.0}_{-0.0}$ & $0.11^{+0.0}_{-0.0}$ \\ \midrule
CAT & $0.94^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.95^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.93^{+0.0}_{-0.0}$ & $0.04^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ \\
        \bottomrule
    \end{tabular}
    \label{tab:trainingsample_high_beambackground}
\end{table*}



The track finding efficiencies for the radiative muon pair events are shown in \cref{fig:kkmc_eff_pt}.
Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate are shown in \cref{tab:kkmc_low_beambackground} and \cref{tab:kkmc_high_beambackground}.


\cref{fig:p_eff_muonpair}

\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/kkmc/ep3/truth_pt_th_0_35_4_hnum_7_1000__efficiency.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/kkmc/ep3/truth_pt_th_35_4_123_4_hnum_7_1000__efficiency.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/kkmc/ep3/truth_pt_th_123_4_180_hnum_7_1000__efficiency.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c}
     \end{subfigure}\hfill\\
     
      \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/kkmc/np3/truth_pt_th_0_35_4_hnum_7_1000__efficiency.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/kkmc/np3/truth_pt_th_35_4_123_4_hnum_7_1000__efficiency.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/kkmc/np3/truth_pt_th_123_4_180_hnum_7_1000__efficiency.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c2}
     \end{subfigure}

\caption{Track finding~(empty markers) and combined track finding and fitting efficiency~(filled markers) for radiative muon pair events. See \cref{fig:p_eff} for details.}
\label{fig:kkmc_eff_pt}
\end{figure*}

\tf{tabelle(n)?}

\begin{table*}
    \fontsize{8pt}{8pt}\selectfont
    \centering
    \caption{Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate for the \kkmc evaluation samples for different track finding algorithms in different detector regions for low beam background. }
    \begin{tabular}{r ccc ccc ccc}
         \toprule
         & \multicolumn{3}{c}{FWD} &  \multicolumn{3}{c}{Barrel} & \multicolumn{3}{c}{BWD} \\
         & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate\\
         \midrule

        Legendre & $0.87^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $1.0^{+0.0}_{-0.0}$ & $0.03^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.73^{+0.01}_{-0.01}$ & $0.04^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
CA + Legendre & $0.94^{+0.0}_{-0.0}$ & $0.1^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $1.0^{+0.0}_{-0.0}$ & $0.05^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.95^{+0.0}_{-0.0}$ & $0.13^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
CA & $0.95^{+0.0}_{-0.0}$ & $0.16^{+0.0}_{-0.0}$ & $0.05^{+0.0}_{-0.0}$ & $1.0^{+0.0}_{-0.0}$ & $0.08^{+0.0}_{-0.0}$ & $0.13^{+0.0}_{-0.0}$ & $0.96^{+0.0}_{-0.0}$ & $0.18^{+0.0}_{-0.0}$ & $0.04^{+0.0}_{-0.0}$ \\ \midrule
CAT & $0.97^{+0.0}_{-0.0}$ & $0.09^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $1.0^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.1^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
        \bottomrule
    \end{tabular}
    \label{tab:kkmc_low_beambackground}
\end{table*}


\begin{table*}
    \fontsize{8pt}{8pt}\selectfont
    \centering
    \caption{Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate for the \kkmc evaluation samples for different track finding algorithms in different detector regions for low beam background. }
    \begin{tabular}{r ccc ccc ccc}
         \toprule
         & \multicolumn{3}{c}{FWD} &  \multicolumn{3}{c}{Barrel} & \multicolumn{3}{c}{BWD} \\
         & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate\\
         \midrule

        Legendre & $0.48^{+0.01}_{-0.01}$ & $0.05^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.98^{+0.0}_{-0.0}$ & $0.09^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.31^{+0.01}_{-0.01}$ & $0.17^{+0.01}_{-0.01}$ & $0.0^{+0.0}_{-0.0}$ \\
CA + Legendre & $0.77^{+0.0}_{-0.0}$ & $0.75^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.16^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.76^{+0.0}_{-0.0}$ & $0.78^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ \\
CA & $0.9^{+0.0}_{-0.0}$ & $0.77^{+0.0}_{-0.0}$ & $0.17^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.32^{+0.0}_{-0.0}$ & $0.39^{+0.0}_{-0.0}$ & $0.83^{+0.0}_{-0.0}$ & $0.79^{+0.0}_{-0.0}$ & $0.11^{+0.0}_{-0.0}$ \\ \midrule
CAT & $0.95^{+0.0}_{-0.0}$ & $0.21^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.99^{+0.0}_{-0.0}$ & $0.09^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.96^{+0.0}_{-0.0}$ & $0.4^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ \\
        \bottomrule
    \end{tabular}
    \label{tab:kkmc_high_beambackground}
\end{table*}

The track finding efficiencies for prompt tracks in $B^+B^-$ events are shown in \cref{fig:bb_eff_pt}.
Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate are shown in \cref{tab:bb_low_beambackground} and \cref{tab:bb_high_beambackground}.

\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/b_decays/ep3/truth_pt_vrho_0_0_5_vrho__2_2_hnum_7_1000_th_0_35_4__efficiency.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/b_decays/ep3/truth_pt_vrho_0_0_5_vrho__2_2_hnum_7_1000_th_35_4_123_4__efficiency.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/b_decays/ep3/truth_pt_vrho_0_0_5_vrho__2_2_hnum_7_1000_th_123_4_180__efficiency.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c}
     \end{subfigure}\hfill\\
     
      \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/b_decays/np3/truth_pt_vrho_0_0_5_vrho__2_2_hnum_7_1000_th_0_35_4__efficiency.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/b_decays/np3/truth_pt_vrho_0_0_5_vrho__2_2_hnum_7_1000_th_35_4_123_4__efficiency.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/prompt_results/b_decays/np3/truth_pt_vrho_0_0_5_vrho__2_2_hnum_7_1000_th_123_4_180__efficiency.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c2}
     \end{subfigure}

\caption{Track finding~(empty markers) and combined track finding and fitting efficiency~(filled markers) for prompt tracks in $B^+ B^-$ events. See \cref{fig:p_eff} for details.}
\label{fig:bb_eff_pt}
\end{figure*}

\begin{table*}
    \fontsize{8pt}{8pt}\selectfont
    \centering
    \caption{Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate for the \charged evaluation samples for different track finding algorithms in different detector regions for low beam background. }
    \begin{tabular}{r ccc ccc ccc}
         \toprule
         & \multicolumn{3}{c}{FWD} &  \multicolumn{3}{c}{Barrel} & \multicolumn{3}{c}{BWD} \\
         & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate\\
         \midrule
        Legendre & $0.73^{+0.0}_{-0.0}$ & $0.54^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.93^{+0.0}_{-0.0}$ & $0.58^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.65^{+0.0}_{-0.0}$ & $0.58^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
CA + Legendre & $0.86^{+0.0}_{-0.0}$ & $0.69^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.94^{+0.0}_{-0.0}$ & $0.61^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.84^{+0.0}_{-0.0}$ & $0.73^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ \\
CA & $0.88^{+0.0}_{-0.0}$ & $0.68^{+0.0}_{-0.0}$ & $0.08^{+0.0}_{-0.0}$ & $0.96^{+0.0}_{-0.0}$ & $0.64^{+0.0}_{-0.0}$ & $0.28^{+0.0}_{-0.0}$ & $0.85^{+0.0}_{-0.0}$ & $0.7^{+0.0}_{-0.0}$ & $0.06^{+0.0}_{-0.0}$ \\
CAT & $0.42^{+0.0}_{-0.0}$ & $0.51^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.55^{+0.0}_{-0.0}$ & $0.5^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.42^{+0.0}_{-0.0}$ & $0.57^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ \\
        \bottomrule
    \end{tabular}
    \label{tab:bb_low_beambackground}
\end{table*}

\begin{table*}
    \fontsize{8pt}{8pt}\selectfont
    \centering
    \caption{Track finding efficiency \trackeff, fake rate \fakerate, and clone rate \clonerate for the \charged evaluation samples for  different track finding algorithms in different detector regions for high beam background. }
    \begin{tabular}{r ccc ccc ccc}
         \toprule
         & \multicolumn{3}{c}{FWD} &  \multicolumn{3}{c}{Barrel} & \multicolumn{3}{c}{BWD} \\
         & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate & \trackeff & \fakerate & \clonerate\\
         \midrule

Legendre & $0.48^{+0.0}_{-0.0}$ & $0.51^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.88^{+0.0}_{-0.0}$ & $0.57^{+0.0}_{-0.0}$ & $0.0^{+0.0}_{-0.0}$ & $0.38^{+0.0}_{-0.0}$ & $0.6^{+0.01}_{-0.01}$ & $0.0^{+0.0}_{-0.0}$ \\
CA + Legendre & $0.72^{+0.0}_{-0.0}$ & $0.81^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.9^{+0.0}_{-0.0}$ & $0.6^{+0.0}_{-0.0}$ & $0.02^{+0.0}_{-0.0}$ & $0.66^{+0.0}_{-0.0}$ & $0.86^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ \\
CA & $0.79^{+0.0}_{-0.0}$ & $0.75^{+0.0}_{-0.0}$ & $0.13^{+0.0}_{-0.0}$ & $0.94^{+0.0}_{-0.0}$ & $0.65^{+0.0}_{-0.0}$ & $0.41^{+0.0}_{-0.0}$ & $0.73^{+0.0}_{-0.0}$ & $0.77^{+0.0}_{-0.0}$ & $0.09^{+0.0}_{-0.0}$ \\ \midrule
CAT & $0.4^{+0.0}_{-0.0}$ & $0.56^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.51^{+0.0}_{-0.0}$ & $0.53^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ & $0.36^{+0.0}_{-0.0}$ & $0.62^{+0.0}_{-0.0}$ & $0.01^{+0.0}_{-0.0}$ \\
        \bottomrule
    \end{tabular}
    \label{tab:bb_high_beambackground}
\end{table*}



\FloatBarrier
\subsubsection{Displaced tracks}
\cref{fig:p_eff_darkhiggs}

\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example_2d.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example_2d.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example_2d.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c}
     \end{subfigure}\hfill\\
     
      \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example_2d.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example_2d.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example_2d.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c2}
     \end{subfigure}

\caption{Track finding~(empty markers) and combined track finding and fitting efficiency~(filled markers) for $h\to\mu^+\mu^-$ events. .}
\label{fig:p_eff_darkhiggs}
\end{figure*}

\begin{figure*}[ht!]
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         \caption{Forward endcap.}
         \label{fig:p_eff:a}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         \caption{Barrel.}
         \label{fig:p_eff:b}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{example-image-a}
         \caption{Backward endcap.}
         \label{fig:p_eff:c}
     \end{subfigure}\hfill\\
     
      \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/displaced_results/b_to_jpsi_kshort/CAT Fitterth_0_35_4_motherpdg_309_5_310_5_efficiency_truth_pt_truth_vrho_2d_imshow.pdf}
         \caption{Forward endcap.}
         \label{fig:p_eff:a2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/displaced_results/b_to_jpsi_kshort/CAT Fitterth_35_4_123_4_motherpdg_309_5_310_5_efficiency_truth_pt_truth_vrho_2d_imshow.pdf}
         \caption{Barrel.}
         \label{fig:p_eff:b2}
     \end{subfigure}\hfill
        \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/displaced_results/b_to_jpsi_kshort/CAT Fitterth_123_4_180_motherpdg_309_5_310_5_efficiency_truth_pt_truth_vrho_2d_imshow.pdf}
         \caption{Backward endcap.}
         \label{fig:p_eff:c2}
     \end{subfigure}

\caption{Track finding~(empty markers) and combined track finding and fitting efficiency~(filled markers) for $h\to\mu^+\mu^-$ events. .}
\label{fig:p_eff_dks_bksjpsi}
\end{figure*}
\tf{tabelle(n)?}

\tf{for displaced (dark higgs), we need 2D plots, x-axis always displacement - is stat high enough?}\\
\tf{tabellen}



\tf{not trained on: Same plots for K0S from B events}\\
\tf{Discuss events that are found and not-found by the different TFs.}\\
\tf{discuss results}\\

\subsection{Track momentum and position resolution}\label{sec_results_momentum}
\tf{use tracking paper definition}
\tf{same plots as for efficiency for pt, p, pz}
\tf{position nach finding nur \cat}

\subsection{Beam Background Robustness}\label{sec_results_beambackground}
\tf{How does the model perform during inference for (slightly) changed beam background conditions?}

\subsection{Generalisation performance}\label{sec_results_generalization}
\tf{How does the model perform during inference for events with more tracks than it has seen during training?}
\tf{test electrons and/or pions}

\subsection{Performance}\label{sec-time}
\tf{inference time and memory consumption (if we have an interface that is a somewhat competitive)?}






% \textcolor{red}{LEA+TORBEN+SALLY: Particle gun performance as function of number of tracks, pt, theta, beam background level. Discuss hyperparameter optimization (incl. optimization of beta). Discuss robustness against beam background, against unlearned number of tracks, against unlearned pt range etc}

%Sally
%Order: definitions: evaluations and predictions

%Sally 
%Main messages to be described:
%\begin{itemize}
%\item Soft $p_{T}$ tracks are outperforming basf2 reco by x\% 
%\item Theta to see the bias in z
%\item How often do we classify beam background hit
%\item Beam background tracks with 10\% bkg luminosity  wrt basf2 (maybe for this we need higher lumi  bkg)
%\item Typical Belle II number of tracks in event is not confusing our algorithm
%\item 
% \color{black}
%\end{itemize}
%
% The baseline \textit{basf2} tracking algorithm is based on xx is used as a comparison for the GNN-based algorithm. 
% There are three features of the \textit{basf2} tracking algorithm which are non-optimal. Firstly, this algorithm is optimised for tracks originating from interaction point, as most of the particles in $B$-meson decays will originate from there. 
% There are, however, Standard Model particles with longer lifetimes, such as $\Lambda$ and $K^{0}_{s}$, with significantly displaced vertexes. Moreover, BSM mediator candidates can have longer lifetimes \cite{}. Secondly, the \textit{basf2} tracking algorithm is not yet optimized for high \textit{beam backgrounds}. Thirdly the \textit{basf2} tracking algorithm is not fully efficient for low transverse momentum ($p_{T}$) tracks. All of these features are addressed by novel GNN-based algorithm.

% In the following section track objects as defined by trigger, \textit{basf2} tracking algorithm, and GNN-based algorithm are compared. Tracks object in trigger is defined as xx [add reference]. Track objects from \textit{basf2} tracking algorithm are objects provided by tracking chain described in [add reference]. In order to make fair comparison track objects after step zz are compared. 




% In this section main findings are described.
% \subsection{Track-finding Efficiency}
% Track-finding efficiency is defined as the efficiency to find a given track in the event by an algorithm, which satisfies the following \textit{matching} criteria: the hit purity for the track must exceeds 66\% and hit efficiency must be above 5\%.
% In~\autoref{fig:p_eff}, ~\autoref{fig:pt_eff}, ~\autoref{fig:pt_eff}, ~\autoref{fig:phi_eff}, ~\autoref{fig:theta_eff}, ~\autoref{fig:vrho_eff}, ~\autoref{fig:ntracks_eff}, the track efficiency as a function of different track- and vertex- properties. The GNN-based track efficiency is 80\% and mostly constant as a function of these variables. It outperforms significantly efficiency of the trigger and the \textit{basf2} tracking algorithm, which is 20\% and 60\% respectively.

% \subsection{Tracking Performance}
% In order to be able to have efficient and ideally performing tracking, the tracking algorithms should minimize spurious tracks, tracks that do not satisfy the \textit{matching} criteria. First class of such tracks are \textit{fake tracks}. They are created by random combinations of hits or by combination of hits originating from two different particles. Second class of the spurious tracks, \textit{clones}, are tracks which were identified several times. The aim is to maximise the the track finding efficiency and minimise the fake and clone track rate. The performance and comparison between the different algorithms is summarised in~\autoref{tab:perf}.


% \subsection{GNN-based Predictions}
% The GNN-based algorithm was trained to predict following track- and vertex- parameters: number of tracks in the event, momentum along $x-,y-,z-$ direction, and the position of the production vertex. The obtained resolutions are shown in~\autoref{fig:pt_res},~\autoref{fig:pz_res},~\autoref{fig:vrho_res},~\autoref{fig:vrho_res} as a function of $p_{T}$, $p_{z}$, $v_{\rho}$. When compared to the resolutions obtained by trigger algorithm, shown in~\autoref{fig:res_comp} the GNN-based algorithm provides much better track estimates that outperform the trigger algorithm by uu\%.




% see Table\,\ref{tab1}
% see Fig.\,\ref{fig1}

% \begin{table}[h]
% \begin{center}
% \begin{minipage}{174pt}
% \caption{Performance of different track-finding algorithms. Evaluation is performed on the zz samples. GNN-based algorithm is the most efficient algorithm. }\label{tab1}%
% \begin{tabular}{@{}llll@{}}
% \toprule
% Track & GNN-based  & Trigger & \textit{basf2} Tracking\\
% \midrule
% Efficiency    & 97.1\%   & 26.7\%  & 64.4\%  \\
% Fake Rate   & 2.5\%  & 0.0\%  & 8.7\%  \\
% Clone Rate   & 1.1\%   & 0.1\% 8  & 1.7\%  \\
% \botrule
% \end{tabular}
% \label{tab:perf}
% \end{minipage}
% \end{center}
% \end{table}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackEfficiencyDummy/efficiencies_per_track_p.pdf}
% \caption{Single track efficiency as a function generated $p$ in \color{violet} samples\color{black}\ computed for track objects from GNN based, trigger and \textit{basf2} tracking algorithm. Computed error is statistical.}
% \label{fig:p_eff}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackEfficiencyDummy/efficiencies_per_track_pt.pdf}
% \caption{Single track efficiency as a function generated $p_{T}$ in \color{violet} samples\color{black}\ computed for track objects from GNN based, trigger and \textit{basf2} tracking algorithm. Computed error is statistical.}
% \label{fig:pt_eff}
% \end{figure}


% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackEfficiencyDummy/efficiencies_per_track_phi.pdf}
% \caption{Single track efficiency as a function generated $\phi$ in \color{violet} samples\color{black}\ computed for track objects from GNN based, trigger and \textit{basf2} tracking algorithm. Computed error is statistical.}
% \label{fig:phi_eff}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackEfficiencyDummy/efficiencies_per_track_theta.pdf}
% \caption{Single track efficiency as a function generated $\theta$ in \color{violet} samples\color{black}\ computed for track objects from GNN based, trigger and \textit{basf2} tracking algorithm. Computed error is statistical.}
% \label{fig:theta_eff}
% \end{figure}


% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackEfficiencyDummy/efficiencies_per_track_vrho.pdf}%
% \caption{Single track efficiency as a function generated displacement, $v_{\rho}$, from the interaction point in \color{violet} samples\color{black}\ computed for track objects from GNN based, trigger and \textit{basf2} tracking algorithm. Computed error is statistical.}
% \label{fig:vrho_eff}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackEfficiencyDummy/efficiencies_per_track_n_tracks.pdf}
% \caption{Single track efficiency as a function generated number of tracks in the event in \color{violet} samples\color{black}\ computed for track objects from GNN based, trigger and \textit{basf2} tracking algorithm. Computed error is statistical.}
% \label{fig:ntracks_eff}
% \end{figure}


% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackResolutionDummy/rel_pt_resolution_tracks.pdf}
% \caption{ Relative $p_{T}$ resolution, $\frac{p^{predicted}_{T}-p^{truth}_{T}}{p^{truth}}$, for displaced tracks reaches 20\% .}
% \label{fig:pt_res}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackResolutionDummy/rel_pz_resolution_tracks.pdf}
% \caption{ Relative $p_{z}$ resolution, $\frac{p^{predicted}_{z}-p^{truth}_{z}}{p^{truth}}$, is expectantly worse but reached globally 25\%.}
% \label{fig:pz_res}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackResolutionDummy/rel_pos_resolution_tracks.pdf}
% \caption{$v_{\rho}$ resolution, $v^{\rho}_{predicted}-v^{\rho}_{truth}$, is 2.5 cm \% .}
% \label{fig:vrho_res}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/TrackResolutionDummy/rel_pz_resolution_tracks.pdf}
% \caption{$v_{z}$ resolution, $v^{z}_{predicted}-v^{z}_{truth}$, is worse than $v_{\rho}$ resolution but it is well below 10 cm.}
% \label{fig:vz_res}
% \end{figure}



% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.2\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/TrackResolutionDummy/rel_phi_resolution_tracks.pdf}
%          \caption{$\phi$}
%          \label{fig:phi_res}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.2\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/TrackResolutionDummy/rel_theta_resolution_tracks.pdf}
%          \caption{$\theta$}
%          \label{fig:theta_res}
%      \end{subfigure} \\
%      \hfill
%         \caption{Prediction Histogram Plots}
%         \label{fig:res}
        
% \end{figure}



% \begin{figure}[h]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/example_displaced_efficiencies_per_track_vr.pdf}
% \caption{Comparison of track reconstruction efficiency between \textit{basf2} (orange), trigger (blue) and GNN-based algorithm (red) as a function of displacement $\rho^{MC}_{h^{'}}$ for the same events. GNN based algorithm track efficiency is constant and above 70\%, whereas trigger and \textit{basf2} algorithm decrease linearly. Track efficiency below 17 cm are not comparable as the GNN based algorithm does not use infromation from SVD and PXD.}\label{fig3}
% \end{figure}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/example_comparison_pt_particles.pdf}
% \caption{20\% resolution for $p_{T}$ obtained from GNN based algorithm (red) is much improved compared to the resolution of trigger (blue) algorithm.}
% \label{fig:res_comp}
% \end{figure}

